Inverse-Compton drag on a Highly Magnetized GRB jet in Stellar Envelope

The collimation and evolution of relativistic outflows in $\gamma$-ray bursts (GRBs) are determined by their interaction with the stellar envelope through which they travel before reaching the much larger distance where the energy is dissipated and $\gamma$-rays are produced. We consider the case of a Poynting flux dominated relativistic outflow and show that it suffers strong inverse-Compton (IC) scattering drag near the stellar surface and the jet is slowed down to sub-relativistic speed if its initial magnetization parameter ($\sigma_0$) is larger than about 10$^5$. If the temperature of the cocoon surrounding the jet were to be larger than about 10 keV, then an optically thick layer of electrons and positrons forms at the interface of the cocoon and the jet, and one might expect this pair screen to protect the interior of the jet from IC drag. However, the pair screen turns out to be ephemeral, and instead of shielding the jet it speeds up the IC drag on it. Although a high $\sigma_0$ jet might not survive its passage through the star, a fraction of its energy is converted to 1-100 MeV radiation that escapes the star and appears as a bright flash lasting for about 10 s.

==> fig-jet-shells.tex <==
 %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[scale=1]
\shadedraw[left color=white, right color=yellow!15!white,draw=none](0,0) --node[below, sloped, very near end,font=\bfseries, color=gray!70!white]{star envelope} +(30:9) arc(30:-30:16.5 and 9) -- cycle;
\shadedraw[left color=cyan!30!white, right color=blue!40!cyan,draw=none] plot [smooth cycle] coordinates {(0,0) (8,2.5) (10.2,0) (8,-2.5)}; 
\shadedraw[color=red!20!white,left color=red!20!white, right color=red!80!magenta, style=very thin, draw=none]
plot [smooth cycle] coordinates {(0,0) (8,1.55) (10,0) (8,-1.55)};
\shadedraw[color=red!20!white,left color=red!20!white, right color=red!80!magenta, style=very thin, draw=none]
plot [smooth cycle] coordinates {(2,0) (8.5,1.9) (10.05,0) (8.5,-1.9)};
\shadedraw[color=orange!20!white,left color=orange!20!white, right color=orange!50!white, style=very thin, draw=none]
plot [smooth cycle] coordinates {(0,0) (8,1.4) (10,0) (8,-1.4)};
\shadedraw[left color=yellow!20!white, right color=yellow!50!white, style=very thin, draw=none] plot [smooth cycle] coordinates {(0,0) (8,.8) (10,0) (8,-.8)}; 
\begin{scope}[color=black,style=very thick]
\tikzstyle{every node} = [scale=.25,fill=red!70!, circle,text=black,font=\large,font=\bfseries, style=very thick]
\node at (1.8,0.4) {$+$};
\node at (2.5,0.5) {$+$};
\node at (3,0.55) {$+$};
\node at (3.8,0.65) {$+$};
\node at (4,.75) {$+$};
\node at (4.6,.7) {$+$};
\node at (5.2,.9) {$+$};
\node at (5.5,.85) {$+$};
\node at (6.,0.9) {$+$};
\node at (6.5,1.15) {$+$};
\node at (6.7,.9) {$+$};
\node at (7.1,1.05) {$+$};
\node at (7.6,1.0) {$+$};
\node at (8,1.15) {$+$};
\node at (8.3,1) {$+$};
\node at (8.8,1.1) {$+$};
\node at (8.9,.9) {$+$};
\node at (9.25,.85) {$+$};
\node at (9.65,.6) {$+$};
%
\node at (1.8,-0.4) {$+$};
\node at (2.5,-0.5) {$+$};
\node at (3,-0.55) {$+$};
\node at (3.8,-0.65) {$+$};
\node at (4,-.75) {$+$};
\node at (4.6,-.7) {$+$};
\node at (5.2,-.9) {$+$};
\node at (5.5,-1.0) {$+$};
\node at (6.,-0.9) {$+$};
\node at (6.5,-1.2) {$+$};
\node at (6.7,-.9) {$+$};
\node at (7,-1.2) {$+$};
\node at (7.1,-1.05) {$+$};
\node at (7.6,-1) {$+$};
% \node at (7.8,-1.6) {$+$};
% \node at (7.9,-2.) {$+$};
\node at (8,-1.2) {$+$};
% \node at (8.,-1.6) {$+$};
\node at (8.3,-1) {$+$};
\node at (8.8,-1.1) {$+$};
\node at (8.9,-.9) {$+$};
\node at (9.25,-.85) {$+$};
% \node at (9.4,-1.45) {$+$};
\node at (9.6,-.6) {$+$};
% 
\tikzstyle{every node} = [scale=.25,fill=blue!30!white, circle,text=black,font=\large,font=\bfseries, style=very thick]
\node at (1.33,0.35) {$-$};
\node at (2.3,0.45) {$-$};
\node at (2.85,0.5) {$-$};
\node at (3.4,.6) {$-$};
\node at (4.3,.7) {$-$};
\node at (4.7,.9) {$-$};
\node at (5.7,1.1) {$-$};
\node at (5.8,0.8) {$-$};
\node at (6.,1.15) {$-$};
\node at (6.4,0.9) {$-$};
% \node at (6.7,1.6) {$-$};
\node at (8,1.) {$-$};
% \node at (7.2,1.75) {$-$};
\node at (7.4,1.1) {$-$};
\node at (7.8,1.25) {$-$};
% \node at (8,1.6) {$-$};
% \node at (8.3,1.6) {$-$};
\node at (8.4,1.1) {$-$};
% \node at (8.6,2.2) {$-$};
\node at (8.6,1.) {$-$};
\node at (9.05,1.) {$-$};
\node at (9.4,.7) {$-$};
\node at (9.75,.45) {$-$};
%
\node at (1.33,-0.35) {$-$};
\node at (2.3,-0.45) {$-$};
\node at (2.85,-0.5) {$-$};
\node at (3.4,-.6) {$-$};
\node at (4.3,-.7) {$-$};
\node at (4.7,-.9) {$-$};
\node at (5.7,-1.1) {$-$};
\node at (5.8,-0.8) {$-$};
\node at (6.1,-1.1) {$-$};
\node at (6.5,-1.0) {$-$};
\node at (6.7,-1.1) {$-$};
\node at (8.2,-1.2) {$-$};
% \node at (7.2,-1.75) {$-$};
\node at (7.4,-.9) {$-$};
\node at (7.6,-1.2) {$-$};
\node at (7.8,-.9) {$-$};
% \node at (8.3,-1.6) {$-$};
\node at (8.4,-1.15) {$-$};
\node at (8.6,-1.) {$-$};
\node at (9.05,-1.) {$-$};
\node at (9.4,-.7) {$-$};
\node at (9.75,-.45) {$-$};
\end{scope}
\draw (10.5,3) -- (10.2,3) --node[very near start, above=4pt, right=8pt,font=\bfseries] {cocoon} (9.1,1.5);
\draw (10.5,2.5) -- (10.2,2.5) --node[very near start, above=4pt, right=8pt,font=\bfseries] {IC-dragged layer} (9.3,1.1);
\draw (10.5,2) -- (10.2,2) --node[very near start, above=4pt, right=8pt,font=\bfseries] {pairs-layer} (9.5,.7);
\draw (10.5,1.5) -- (10.2,1.5) --node[very near start, above=4pt, right=8pt,font=\bfseries] {jet core} (9.7,.3);
\draw[black, dotted, very thick,->] (0,0)-- (12,0);
\begin{scope}[xshift=-5cm,yshift=1cm]
\pgfsetfillopacity{.8}
\draw[fill=white,style=very thin] (2,-.2)--(5.5,-.2)--(5.5,2)--(2,2)--(2,-.2);
\draw[->,decorate,decoration={snake,amplitude=.5mm,segment length=2.5mm}]
 {(2.7,1.1) -- node[->,very near start, above=-1pt]{$\gamma_{c}$} (3,0.3)};
\node[scale=.3,fill=yellow, circle,text=black,font=\large,font=\bfseries, style=very thick,color=black] at (3.1,.2) {$-$};
\node[scale=.29,fill=yellow, circle,text=black,font=\large,font=\bfseries, style=very thick] at (3.1,.2) {$-$};
\draw[->,decorate,decoration={snake,amplitude=.1mm,segment length=1.5mm}]
 {(3.2,.2) -- node[midway, above]{$\gamma_{ic}$} (4.5,0.2)};
\draw[->,decorate,decoration={snake,amplitude=.5mm,segment length=2.5mm}]
 {(4,1.4) -- node[very near start, above=1pt]{$\gamma_{c}$} (4.5,0.25)};
% \draw[->,black,snake=snake,segment amplitude=.4mm,segment length=2mm,line after snake=1mm] (4,1.1) -- node[very near start, above=1pt]{$\gamma_{c}$} (4.5,0.25);
\draw[->](4.55,0.25) --(4.88,0.65);
\draw[->](4.55,0.2) --(5.15,0.7);
\node[scale=.31,fill=black, color=black,circle] at (4.95,.75) {$+$};
\node[scale=.31,fill=black, color=black,circle] at (5.2,0.8) {$-$};
\node[scale=.3,fill=red!80!, circle,text=black,font=\large,font=\bfseries, style=very thick] at (4.95,.75) {$+$};
\node[scale=.3,fill=blue!60!white, circle,text=black,font=\large,font=\bfseries, style=very thick] at (5.2,0.8) {$-$};
\draw[->,thick] (5.6,.9) -- (9.5,-.2);
\end{scope}
\end{tikzpicture}
